Deconvolved Image Restoration from Autocorrelations

Recovering a signal from auto-correlations or, equivalently, retrieving the phase linked to a given Fourier modulus, is a wide-spread problem in imaging. This problem has been tackled in a number of experimental situations, from optical microscopy to adaptive astronomy, making use of assumptions based on constraints and prior information about the recovered object. In a similar fashion, deconvolution is another common problem in imaging, in particular within the optical community, allowing high-resolution reconstruction of blurred images. Here we address the mixed problem of performing the auto-correlation inversion while, at the same time, deconvolving its current estimation. To this end, we propose an I-divergence optimization, driving our formalism into a widely used iterative scheme, inspired by Bayesian-based approaches. We demonstrate the method recovering the signal from blurred auto-correlations, further analysing the cases of blurred objects and band-limited Fourier measurements.

==> temp.tex <==
\section{Complete variational derivative of $\chi^*$}
As per the definition of variational derivative \cite{Engel2011}, we let the function $o$ variate by a small amount $o + \epsilon \theta$, thus we compute:
\begin{equation}
    \frac{d}{d\epsilon} F \left[ o + \epsilon \theta \right] \bigg|_{\epsilon=0} =: \int \frac{\delta F\left[ o \right]}{\delta \left[ o\left(x \right) \right]} \theta\left(x \right) \,dx
\end{equation}
We have that we need to compute the functional derivative of 
\begin{align}
    \frac{\delta}{\delta \left[ o\left(x \right) \right]} F\left[ o\left(x \right) \right] &= \frac{\delta}{\delta \left[ o\left(x \right) \right]}\left[ \left( o \star o \right) * \mathcal{H}\right] \nonumber \\ 
    &= \bigg\{ \frac{\delta\left( o \star o \right)}{\delta \left[ o\left(x \right) \right]} \bigg\} * \mathcal{H},
\end{align}
since $\mathcal{H}$ does not depend explicitly on $o$. We are left with the calculation of the functional derivative of the auto-correlation function. This can be done by noticing that:
\begin{align}
    \frac{d}{d\epsilon} F & \left[ o + \epsilon \theta \right] \bigg|_{\epsilon=0} = \nonumber \\ &= \frac{d}{d\epsilon} \int \left[ \overline{o(x)} + \epsilon\overline{\theta(x)} \right] \left[ {o(x+\xi)} + \epsilon {\theta(x+\xi)} \right]\bigg|_{\epsilon=0} \,dx \nonumber \\
    &= \frac{d}{d\epsilon} \int \epsilon \left[ \overline{o(x)} \theta(x+\xi) +  o(x+\xi) \overline{\theta(x)}\right]\bigg|_{\epsilon=0} \,dx \nonumber \\
    &= \int \left[ \overline{o(x)} \theta(x+\xi) +  o(x+\xi) \overline{\theta(x)}\right] \,dx \nonumber \\
    &= \int \left[ \overline{o(x-\xi)} \theta(x) +  o(x+\xi) \overline{\theta(x)}\right] \,dx \nonumber \\
    &= \int \left[ {o(x-\xi)} +  o(x+\xi) \right]\theta(x) \,dx
\end{align}
where on the latter we used the fact that in our case the functions are real thus $\overline{f(x)}=f(x)$ and $\overline{\theta(x)}=\theta(x)$.
Thus, we can recognize the functional derivative as a linear operator acting on the test function:
\begin{equation} \label{eq:finalfunctionalderivative}
    \frac{\delta}{\delta \left[ o\left(x \right) \right]}\left[ \chi * \mathcal{H}\right] = \left[ {o(x-\xi)} +  o(x+\xi) \right] * \mathcal{H}
\end{equation} 
A similar result can be found for n-th order correlations in \cite{schulz1992image} and so, our formulation suggests that the convolution with any independent kernel does not play any relevant role in the functional derivative. 
In the special case the function $o$ is hermitian, eq. \ref{eq:finalfunctionalderivative} reduces to:
\begin{equation}
    \frac{\delta}{\delta \left[ o\left(x \right) \right]}\left[ \chi * \mathcal{H}\right] = o\left(x+\xi\right) * \mathcal{H}
\end{equation}

\section{Rigorous iterative method}
By setting to zero and inserting the functional derivative calculated in the appendix, eq. \ref{eq:finalfunctionalderivative}, we obtain:
\begin{equation}\label{eq:integraltozero}
    \int \left(1- \frac{\chi_\mu}{\chi^*\left( \xi \right)} \right) \left[ {o(x-\xi)} +  o(x+\xi) \right] * \mathcal{H} \,d\xi = 0
\end{equation}
A closed solution does not exist in general, however, an efficient scheme to approach the solution of eq. \ref{eq:integraltozero} is given by the Picard iteration \cite{isaacson2012analysis}.
This implies the usage of a fixed-point iterative formulation:
\begin{equation}
    o^{t+1}(x) = o^t (x) \lambda^t(x)
\end{equation}
where
\begin{equation}
    \lambda^t(x) = \int \frac{\chi_\mu\left(\xi\right)}{\int o^{t}\left(x\right) \mathcal{K}^{t}\left(\xi - x\right) \,dx}\left[ {o(x-\xi)} +  o(x+\xi) \right] * \mathcal{H} \,d\xi
\end{equation}
The full expression that leads to optimal results would be:
\begin{align}
    &\mathcal{K}^{t} = o^t \star \mathcal{H} \\
    &o^{t+1} = o^{t} \left[ \left(\frac{\chi_\mu}{o^{t} * \mathcal{K}^{t}}\right)*\widetilde{\mathcal{K}}^{t} + \left(\frac{\chi_\mu}{o^{t} * \mathcal{K}^{t}}\right) \star {\mathcal{K}}^{t}\right]
\end{align}
where $\widetilde{\mathcal{K}}$ denotes reversed axis.

